A coupled lattice Boltzmann model for pore-scale mushy-layer dynamics with application to sea ice

A pore-scale lattice Boltzmann model is developed for reactive transport in phase-changing porous media, coupling solute transport in the liquid with conjugate heat transfer across the solid and liquid phases. Two methodological developments are introduced: a novel link-based Volume-of-Pixel formulation for direction-dependent interface motion, and a generalized Robin boundary treatment for solute redistribution at moving interfaces. The phase-change formulation is validated against thermal benchmarks, while the Robin treatment is assessed through literature test cases, exhibiting convergence rates between first and second order. The coupled model is then applied to a local pore-scale segment of a sea ice brine channel in a purely diffusive regime. The simulations recover the expected ideal mushy-layer behaviour under appropriate scale separation. At sea-ice-relevant concentration ratios, thermal perturbations produce relatively large variations in brine salinity, causing freezing rather than melting to reshape the pore geometry in a non-uniform way. The resulting framework provides a pore-scale numerical tool for resolving coupled temperature, solute redistribution, and phase-boundary dynamics in mushy layers.

==> figures/ring/corner_convex_a2zero/name.tex <==
\begin{tikzpicture}[font=\sffamily\sansmath]

\begin{axis}[
width=\figurewidth,
height=\figureheight,
scale only axis,
xmin=64,
xmax=90,
ymin=64,
ymax=90,
axis equal image,
axis lines=none,
xtick=\empty,
ytick=\empty,
clip=true,
]

% ============================================================
% Lattice connections only between displayed nodes
% ============================================================

\addplot[
gray!70,
solid,
line width=0.42pt,
unbounded coords=jump
]
table[
x index=0,
y index=1
]{figures/ring/corner_convex_a2zero/ring_outer_grid_segments.dat};

% ============================================================
% Solid nodes outside the outer ring boundary:
% hollow black circles
% ============================================================

\addplot[
only marks,
black,
mark=o,
mark size=1.65pt,
mark options={
    solid,
    fill=white,
    draw=black,
    line width=0.65pt
}
]
table[
x index=0,
y index=1
]{figures/ring/corner_convex_a2zero/ring_outer_solid_nodes.dat};

% ============================================================
% Fluid nodes inside the outer ring boundary:
% filled blue circles
% ============================================================

\addplot[
only marks,
blue,
mark=*,
mark size=1.65pt,
mark options={
    solid,
    fill=blue,
    draw=blue,
    line width=0.65pt
}
]
table[
x index=0,
y index=1
]{figures/ring/corner_convex_a2zero/ring_outer_fluid_nodes.dat};

% ============================================================
% Stair-step outer boundary
% ============================================================

\addplot[
black,
solid,
line width=0.90pt,
unbounded coords=jump
]
table[
x=x,
y=z
]{figures/ring/corner_convex_a2zero/ring_boundary.dat};

% ============================================================
% Corrected convex nodes:
% filled red circles
% ============================================================

\addplot[
only marks,
red,
mark=*,
mark size=1.65pt,
mark options={
    solid,
    fill=red,
    draw=red,
    line width=0.65pt
}
]
table[
x index=0,
y index=1
]{figures/ring/corner_convex_a2zero/outer_convex_corner_nodes.dat};

\end{axis}

\end{tikzpicture}
